Discriminative Semantic Transitive Consistency for Cross-Modal Learning

Cross-modal retrieval is generally performed by projecting and aligning the data from two different modalities onto a shared representation space. This shared space often also acts as a bridge for translating the modalities. We address the problem of learning such representation space by proposing and exploiting the property of Discriminative Semantic Transitive Consistency -- ensuring that the data points are correctly classified even after being transferred to the other modality. Along with semantic transitive consistency, we also enforce the traditional distance minimizing constraint which makes the projections of the corresponding data points from both the modalities to come closer in the representation space. We analyze and compare the contribution of both the loss terms and their interaction, for the task. In addition, we incorporate semantic cycle-consistency for each of the modality. We empirically demonstrate better performance owing to the different components with clear ablation studies. We also provide qualitative results to support the proposals.

==> ablation_hyper_supple.tex <==
\section{Ablation of Hyperparameters}
\label{sec:ablation_hyperparameter}
We experimented with wide range of hyperparameters and picked the one that performs best in the val set. We also observe that the performance remains similar for most of the hyperparameters values. We give the results for \texttt{Sentence Pascal} dataset in Tab.~\ref{tab:hyperparameter} below. We observe from the results that the performance is quite stable for different values of the hyperparameters and the results doesn't change significantly. From this observation, we conclude that the approach is not much sensitive to the value of hyperparameters.
\begin{table}[!htbp]
    \centering
    % \resizebox{.9\columnwidth}{!}{
    % \renewcommand{\arraystretch}{0.4}
    \scalebox{1.0}{
    \begin{tabular}{cccc|ccc}
    \hline
    $\alpha$&$\beta$&$\gamma$&$\delta$ & I2T & T2I & Both\\
    \hline \hline
    10.0 & 1.0 & 0.01 &   0.1 & 0.6923 & 0.7092 & 0.7007\\
    10.0 & 1.0 & 0.01 &   0.0 & 0.6959 & 0.7095 & 0.7027\\
    10.0 & 1.0 & 0.01 &   1.0 & 0.6985 & 0.7104 & 0.7044\\
    10.0 & 1.0 & 0.01 &  10.0 & 0.6897 & 0.7028 & 0.6963\\
    \hline
    10.0 & 1.0 & 0.1 &  0.1 & 0.6944 & 0.7087 & 0.7016\\
    10.0 & 1.0 & 0.1 &  0.0 & 0.6954 & 0.7044 & 0.6999\\
    10.0 & 1.0 & 0.1 &  1.0 & 0.6974 & 0.7017 & 0.6996\\
    10.0 & 1.0 & 0.1 & 10.0 & 0.6882 & 0.7045 & 0.6963\\ 
    \hline
    10.0 & 1.0 & 1.0 &  0.1 & 0.6959 & 0.7059 & 0.7009\\
    10.0 & 1.0 & 1.0 &  0.0 & 0.6963 & 0.7021 & 0.6992\\
    10.0 & 1.0 & 1.0 &  1.0 & 0.6989 & 0.7063 & 0.7026\\
    10.0 & 1.0 & 1.0 & 10.0 & 0.6888 & 0.7031 & 0.6959\\
    \hline
    10.0 & 1.0 & 10.0 &  0.1 & 0.6918 & 0.7020 & 0.6969\\
    10.0 & 1.0 & 10.0 &  0.0 & 0.6914 & 0.7065 & 0.6989\\
    10.0 & 1.0 & 10.0 &  1.0 & 0.6938 & 0.7023 & 0.6981\\
    10.0 & 1.0 & 10.0 & 10.0 & 0.6915 & 0.6994 & 0.6954\\
    \hline
    1.0 & 1.0 & 0.01 &   0.1 & 0.6827 & 0.6954 & 0.6890\\
    1.0 & 1.0 & 0.01 &   0.0 & 0.6763 & 0.7082 & 0.6922\\
    1.0 & 1.0 & 0.01 &   1.0 & 0.6856 & 0.6968 & 0.6912\\
    1.0 & 1.0 & 0.01 &  10.0 & 0.6843 & 0.6998 & 0.6920\\
    \hline
    1.0 & 10.0 & 0.01 &   0.1 & 0.6924 & 0.6820 & 0.6872\\
    1.0 & 10.0 & 0.01 &   0.0 & 0.6761 & 0.6812 & 0.6786\\
    1.0 & 10.0 & 0.01 &   1.0 & 0.6640 & 0.6996 & 0.6818\\
    1.0 & 10.0 & 0.01 &  10.0 & 0.6630 & 0.6876 & 0.6753\\
    \hline \hline
    \end{tabular}
    }
    % \vspace{-1 em}
    \caption{Ablation Study: Contribution of different hyperparameter for retrieval in \texttt{Sentence Pascal} dataset}
    \label{tab:hyperparameter}
    % \vspace{-1 em}
\end{table}
